Sdim: A Qudit Stabilizer Simulator

Quantum computers have steadily improved over the last decade, but developing fault-tolerant quantum computing (FTQC) techniques, required for useful, universal computation remains an ongoing effort. Key elements of FTQC such as error-correcting codes and decoding are supported by a rich bed of stabilizer simulation software such as Stim and CHP, which are essential for numerically characterizing these protocols at realistic scales. Recently, experimental groups have built nascent high-dimensional quantum hardware, known as qudits, which have a myriad of attractive properties for algorithms and FTQC. Despite this, there are no widely available qudit stabilizer simulators. We introduce the first open-source realization of such a simulator for all dimensions. We demonstrate its correctness against existing state vector simulations and benchmark its performance in evaluating and sampling quantum circuits. This simulator is the essential computational infrastructure to explore novel qudit error correction as earlier stabilizer simulators have been for qubits.

==> 3.3_stabilizer_codes.tex <==
% \subsection{Qudit stabilizer quantum error correction codes}

% Finally, we review qudit stabilizer codes, which are the broadest class of quantum error correction codes that can be scalably numerically simulated for important properties such as physical error thresholds.

% We consider an \textit{error} to be some $n$-qudit Pauli $E = E_1 \dots E_n$, and its \textit{weight} $\mathrm{wt}(E) = \text{\# of } E_j \neq I$.  An $[[n, k, D]]_d$ quantum code is a certain map $U: \mathbb{C}^{d^k} \to \mathbb{C}^{d^n}$ taking a $d$-dimensional $k$-qudit state $\ket{\psi}$ to an $n$-qudit state $\ket{\overline{\psi}}$, called a \textit{logical qudit} state.
% This map satisfies certain \textit{error-correcting conditions} which are reviewed and studied in many prolific articles \cite{Knill_2000,gottesmanqeccbook,gottesmanhighdim}.
% The defining property of the map is that if $t = \lfloor (D - 1) / 2 \rfloor$, any error $E$ of weight $t$ or lower that occurs on $\ket{\overline{\psi}} = U \ket{\psi}$ can be corrected by a circuit that automatically determines and applies $E^\dagger$ without collapsing $\ket{\overline{\psi}}$.
% Often, we identify a code by the image of $U$ on states $\ket{\psi}$ we are interested in protecting, called the \textit{codespace}.

% We will restrict our attention to \textit{stabilizer codes}, which protect stabilizer states.
% The defining trait of a stabilizer codespace $V$ is that it is the intersection of $n$-qudit states stabilized by $n - k$ Pauli operators $s_1, s_2, \dots, s_{n - k}$, called \textit{codespace generators}.  That is,
% $$V = \left\{ \ket{\overline{\psi}} \in \mathbb{C}^{d^n} \mid s_1 \ket{\overline{\psi}} = s_2 \ket{\overline{\psi}} = \dots = \ket{\overline{\psi}} \right\} $$
% Recovery from error $E$ is determined by measuring generators $s_j$, called the \textit{error syndrome}.
% Once encoded, we operate on $\ket{\bar{\psi}}$ by \textit{logical operators} that transform it in familiar ways, effectively never leaving the encoding.
% For example, $\bar{X} \ket{\bar{0}} = \ket{\bar{1}} = U \ket{1}$.

% There is a striking resemblance between a stabilizer codespace and a stabilizer state, since both are the intersection of the $+1$ eigenvectors of a group of Pauli operators.
% Therefore, the stabilizer tableau is the \textit{native language} by which we study stabilizer codes and their performance under various metrics such as noise threshold and distance~\cite{Gottesman_1998}.

==> 5.4_evaluation.tex <==
\subsubsection{Evaluation of Pauli frame monte carlo simulation performance in the case study}
The time to sample shots of LRB-D in the tableau versus in Cirq is several hundreds of times faster in the former than the latter.  However, we note that tableau shots seem to grow in runtime faster than the Cirq shots do, echoing observations made in Figure \ref{fig:frametimes} for small system sizes.  Nonetheless, the gulf is large enough that anecdotally, the tableau took 90 minutes to reproduce 120 hours of work from Cirq for 5-qutrit LRB-D.  





% \section{Non-prime dimensions}
% The tableau we introduced for prime qudit stabilizer computation does not straightforwardly generalize in non-prime dimensions.  For example, when $d$ is even, Pauli $P = X^{-1} Z^{-1}$ has order $2d$, as $P^d = -I$.  Furthermore, there are circuits of composite dimension for which random measurements are not uniformly random such as $CNOT^2_{0, 1} \left( F_0 \ket{00}\right)$ in $d = 4$.  A formalism to cope with these difficulties was developed in \cite{de_Beaudrap_2013_composite}.  However, the complexity of measurement is tied to being able to find the \textit{Smith Normal Form} of an integer matrix, which can cost $O(n^4)$ time to compute. 

==> A_1_Qudit_Deutsch_Cartoon.tex <==
\onecolumn
\section{Step-by-step illustration of the qudit Deutsch-Jozsa algorithm}\label{appendix:deutsch_cartoon}
\begin{table}[h]
\begin{adjustbox}{angle=0}
\label{demo-table}
\footnotesize
\begin{tabularx}{1\linewidth}{|p{1.5cm}||X|X|X|X|}
\hline 
\textbf{Source code} & \texttt{c = Circuit(2, 3)} & \texttt{c.add\_gate("H", 0)} & \texttt{c.add\_gate("X", 1)} & \texttt{c.add\_gate("H", 1)} 
\\\hline 
\textbf{Gate\newline operation} & Initialization & $\mathcal{F}\otimes I$ & $I\otimes X$ & $I\otimes\mathcal{F}$
\\\hline
\textbf{Gate\newline unitary} & $\begin{bmatrix}1&0&0\\0&1&0\\0&0&1\end{bmatrix}\otimes I$ & $\frac{1}{\sqrt{3}}\begin{bmatrix}1&1&1\\1&\omega&\omega^2\\1&\omega^2&\omega\end{bmatrix}\otimes I$ & $I\otimes\begin{bmatrix}0&0&1\\1&0&0\\0&1&0\end{bmatrix}$ & $I\otimes\frac{1}{\sqrt{3}}\begin{bmatrix}1&1&1\\1&\omega&\omega^2\\1&\omega^2&\omega\end{bmatrix}$
\\\hline
\textbf{Statevector} & $\ket{0}\otimes\ket{0}$ & $\ket{+}\otimes\ket{0}$ & $\ket{+}\otimes\ket{1}$ & $\ket{+}\otimes\ket{\omega}$ \\\hline
\textbf{Stabilizers} &
{\tiny$\begin{array}{rrr}
II&IZ&IZ^2\\
ZI&ZZ&ZZ^2\\
Z^2I&Z^2Z&Z^2Z^2\\
\end{array}$} &
{\tiny$\begin{array}{rrr}
II&IZ&IZ^2\\
X^2I&X^2Z&X^2Z^2\\
XI&XZ&XZ^2\\
\end{array}$} &
{\tiny$\begin{array}{rrr}
II&I\omega^2Z&I\omega Z^2\\
X^2I&X^2\omega^2Z&X^2\omega Z^2\\
XI&X\omega^2Z&X\omega Z^2\\
\end{array}$} &
{\tiny$\begin{array}{rrr}
II&I\omega^2X^2&I\omega X\\
X^2I&X^2\omega^2X^2&X^2\omega X\\
XI&X\omega^2X^2&X\omega X\\
\end{array}$}
\\\hline
\textbf{Destabilizer generators} & $\{XI,IX\}$ & $\{ZI,IX\}$ & $\{ZI,IX\}$ & $\{ZI,IZ\}$ \\\hline
\textbf{Stabilizer generators} & $\{ZI,IZ\}$ & $\{X^2I,IZ\}$ & $\{X^2I,\omega^2IZ\}$ & $\{X^2I,\omega^2IX^2\}$ \\\hline
\textbf{Tableau} &
$\left[\begin{array}{cc|cc|c}1&0&0&0&0\\0&1&0&0&0\\\hline0&0&1&0&0\\0&0&0&1&0\\\end{array}\right]$ & 
$\left[\begin{array}{cc|cc|c}\underline{0}&0&\underline{1}&0&0\\0&1&0&0&0\\\hline\underline{2}&0&\underline{0}&0&0\\0&0&0&1&0\\\end{array}\right]$ &
$\left[\begin{array}{cc|cc|c}0&0&1&0&0\\0&\underline{1}&0&\underline{0}&0\\\hline2&0&0&0&0\\0&\underline{0}&0&\underline{1}&\underline{2}\\\end{array}\right]$ &
$\left[\begin{array}{cc|cc|c}0&0&1&0&0\\0&\underline{0}&0&\underline{1}&0\\\hline2&0&0&0&0\\0&\underline{2}&0&\underline{0}&2\\\end{array}\right]$
\\\hline
\textbf{Notes} &
Destabilizers $X_i$ on top and stabilizers $Z_i$ on bottom, by convention.&
Note that application of $H$ switches corresponding $X$ and $Z$ columns, which is expected since $H$ changes the $Z$ basis into the $X$ basis. &
Notice there is no change in the Pauli power blocks, but only the phases block because Pauli anticommute with each other. 
&
Same as second step.
\\\hline
\end{tabularx}
\label{table:deutsch-table}
\end{adjustbox}
\end{table}


\twocolumn




==> A_2_Prime_Measurement_is_Gaussian_Elim.tex <==
\section{Prime dimension measurement reduces to Gaussian elimination}\label{appendix:prime_measurement}

Consider tableau $A$ for state $\ket{\psi}$ \textit{without} its destabilizer generators, where we regard it as a matrix over $\mathbb{F}_d$:

\begin{align*}
    A = \left[ \begin{array}{ccc|ccc|c}
        x_{1, 1} & \dots & x_{1, n} & z_{1, 1} & \dots & z_{1, n} & r_1 \\
        \vdots & \ddots & \vdots & \vdots & \ddots & \vdots & \vdots \\
        x_{n, 1} & \dots & x_{n, n} & z_{n, 1} & \dots & z_{n, n} & r_n \\ 
        \end{array} \right]
        =
        \begin{bmatrix}
            --g_1 -- \\
            \vdots \\
            -- g_n --
        \end{bmatrix}
\end{align*}

In order to perform a $Z_j$ measurement, we first ask whether $Z_j$ is in the stabilizer group $S(\ket{\psi})$.  If so, then the following equation has a solution via an assignment to variables $y_1, \dots, y_n$:
\[
Z_j = \omega^l \prod_{j = 1}^n g_j^{y_j}
\]
where $l \in \{0, \dots, d - 1\}$.  If there is a solution, then by definition $\omega^{-l} Z_j \in S(\ket{\psi})$.  On the other hand, if no solution exists, then $\ket{\psi}$ is not an eigenstate of $Z_j$, and the measurement outcome is random.  We can formulate this as a linear algebra problem.  Let:
\[
\Vec{y} = \begin{bmatrix}  y_1, y_2, \dots, y_n\end{bmatrix}^\intercal \in \mathbb{F}_d^{n}
\] 
and write our measurement operator $Z_j$ in the generator encoding:
\[
\Vec{z_j} = 
\begin{bmatrix}  
0, \dots, 0 \mid 0, \dots 1, \dots, 0 \mid 0
\end{bmatrix}^\intercal 
= e_{n + j}^\intercal \in \mathbb{F}_d^{2n + 1}
\]
Now, the following:
\[
A^\intercal \Vec{y} = \Vec{z_j}
\]
is an encoding of our first problem.  We can easily solve this by performing Gaussian elimination on the augmented matrix:
\[
\left[ \begin{array}{c|c} 
    A^\intercal & z_j
\end{array} \right]
\]
Let $B = \text{rref} \left(A \right)$.  After Gaussian elimination, our augmented system looks like: 
\[
\left[ \begin{array}{c|c} 
    B^\intercal & z'
\end{array} \right]
\]
If this form gives us a solution to the $y_j$ variables, then our outcome is deterministically $-l$, as $\ket{\psi}$ is an $\omega^{-l}$-eigenstate of $Z_j$ (or equivalently, $\omega^{-l} Z_j$ stabilizes $\ket{\psi}$).  We can naively solve for $-l$ by directly computing $\prod_{j = 1}^n g_j^{y_j} = \omega^{-l} Z_j$.  

If the form provides no solution, $B$ still gives us the relevant information to perform the random measurement.  For any $a, b \in \{1, \dots, n\}$, notice that $g_a g_b \in S(\ket{\psi})$ and $g_a^k \in S(\ket{\psi})$, where $k \in \{0, \dots, d - 1\}$.  These operations correspond exactly to the steps in Gaussian elimination, so this tells us that
\[
    B =
    \begin{bmatrix}
        -- g'_1 -- \\
        \vdots \\
        -- g'_n --
    \end{bmatrix}
\]

is still a tableau for $\ket{\psi}$.  However, each $g'_j$ acts on mutually exclusive qudits.  For example, if $g'_j = Z_1 Z_2$, then \textit{no other} generator in $B$ is made of (non-identity) operators that act on qudits 1 and 2.  Since this measurement is random, there must be a unique generator $g'_q$ that includes a power of $X_j$.  Replacing $g'_q$ with $\omega^r Z_j$, where $r \in \{0, \dots, d - 1\}$ is random, gives us a tableau for our post-measurement state.  Of course, our measurement outcome was $r$.

For $d = 2$, evaluating $\prod_{j = 1}^n g_j^{y_j}$ may involve multiplying powers of the imaginary unit $i$, and the rowsum protocol in \cite{Aaronson_2004} exactly tracks those contributions to the phase calculation.  However, this technical detail does not appear for odd prime $d$ \cite{gottesmanhighdim}.  

==> A_3_Non-Prime_Tableau.tex <==
\section{Non-prime stabilizer tableau simulation}\label{appendix:non-prime-tableau}


The tableau we introduced for prime qudit stabilizer computation does not cleanly generalize for non-prime dimensions.  For example, when $d$ is even, Pauli $P = X^{-1} Z^{-1}$ has order $2d$, as $P^d = -I$.  These differences manifest both during and after measurement; while $d = 2$ is prime, we observe that as an even dimension, deterministic measurements are more difficult due to factors of $i$ coming out in the phase.  

A formalism to cope with these difficulties was developed in \cite{de_Beaudrap_2013_composite}.  Here, we will outline the essential differences from the prime case.  All difficulties arise from the even cases, so we will assume that $d > 2$ is even. 

\subsection{Representation of non-prime stabilizer generators}

The essential difference between the prime and non-prime cases is the \textit{power of $d$} that show up in the phases of the stabilizer.  This is seen most simply again when $d = 2$, where $i$, a 4th of unity, appears in the phases.  To deal with this, we represent a Pauli stabilizer $Z^a X^b$ as a \textit{Weyl operator} $W_{a, b} = \tau^{-ab} Z^a X^b$, where $\tau = \exp \left((i \pi (d^2 + 1)) / d\right)$.  We can extend this to a product $Z^{a_1}X^{b_1} \otimes \dots \otimes Z^{a_n}X^{b_n}$ by writing:
\[
W_{\Vec{a}, \Vec{b}} = \tau^{- \Vec{a} \cdot \Vec{b}} (Z^{a_1} \otimes \dots \otimes Z^{a_n})(X^{b_1} \otimes \dots \otimes X^{b_n})
\]
where $\Vec{a} = [a_1, \dots, a_n ]$, $\Vec{b} = [b_1, \dots, b_n ]$, and $\Vec{a} \cdot \Vec{b}$ is the dot product.  While this helps us deal with the factors of $d^2$, we still have problems where $W_{0, 1} = - W_{d, 1}$ when $d$ is even, but this cannot be true since $W_{d, 1}$ is non-zero.  The second modification is to lift all our our modular arithmetic to $d'$, which is simply $d$ when $d$ is odd and $2d$ when $d$ is even.  With these modifications in mind, our Weyl operators all have order $d'$.

\subsection{Operations in the non-prime dimension qudit stabilizer tableau}

We do not track any generalization of destabilizer generators, which just leaves with $X$, $Z$, and phase blocks, which encode the integers defining $W_{\Vec{a}, \Vec{b}}$.  Here, we have $2n$ such operators $W_{\Vec{a_1}, \Vec{b_1}}, \dots, W_{\Vec{a_{2n}}, \Vec{b_{2n}}}$.  Note that each $\Vec{a_k}$ is a vector of numbers, and the $j^{\text{th}}$ entry of $\Vec{a_k}$ is $a_{j, k}$.  The same applies to the $b$ variables.
In practice, it is most useful to write the tableau with the Weyl operators stacked from left to right:

\begin{align*}
    \ket{\psi} = 
        \left[ \begin{array}{ccc}
        \tau^{- \Vec{a_1} \cdot \Vec{b_1}} & \dots & \tau^{- \Vec{a_{2n}} \cdot \Vec{b_{2n}}} \\
            \hline \\
            a_{1, 1} & \dots & a_{1, 2n}\\
            \dots & \dots & \dots \\
            a_{n, 1} & \dots & a_{n, 2n} \\
            \hline \\
            b_{1, 1} & \dots & b_{1, 2n}\\
            \dots & \dots & \dots \\
            b_{n, 1} & \dots & b_{n, 2n} \\
        \end{array} \right]
\end{align*}

Consequently, the blocks are stacked by phase, $Z$, and $X$, from top to bottom.
Operating on this tableau via Clifford gates is nearly identical to the prime case in the sense that the conjugations are the same, but they now correspond to rewrite rules on \textit{rows} of the tableau instead of columns.

\subsection{Measurement in the non-prime dimension qudit stabilizer tableau}

We wrote the tableau earlier in an odd fashion since this form, when regarded as a matrix $A$ over $\mathbb{Z}_d$, allows us to reduce the problem of determining measurement outcomes by computing a normal form as in the prime case.  However, $\mathbb{Z}_d$ is no longer guaranteed to be a field when $d$ is an even, non-prime number, so we cannot use Gaussian elimination.  Instead, we use the \textit{Smith normal form} (SNF) of $A$ that expresses it as $USV$, where $U, V$ are invertible and $S$ is a diagonal matrix.  

A key feature of the procedure is that random $Z$ measurements might not be uniformly random over all possible eigenvalues of $Z$.  
%For example, such a measurement outcome for $d = 18$ might only take values randomly from support $\{0, 3, 6, \dots, 15 \}$ \selfnote{Fact check this}. 
 While the Weyl operators are the most general way to represent tableaus of arbitrary dimension, in practice they are incredibly expensive to compute with due to the practical inefficiencies of SNF algorithms on large matrices.  Regrettably, the current build non-prime tableau simulation is often beaten by statevector simulation.

==> A_4_Non-Prime_Measurement_is_SNF.tex <==
\section{Composite dimension measurement reduces to computing Smith normal form}\label{appendix:SNF}
